A Decomposition of Forecast Error in Prediction Markets

We analyze sources of error in prediction market forecasts in order to bound the difference between a security's price and the ground truth it estimates. We consider cost-function-based prediction markets in which an automated market maker adjusts security prices according to the history of trade. We decompose the forecasting error into three components: sampling error, arising because traders only possess noisy estimates of ground truth; market-maker bias, resulting from the use of a particular market maker (i.e., cost function) to facilitate trade; and convergence error, arising because, at any point in time, market prices may still be in flux. Our goal is to make explicit the tradeoffs between these error components, influenced by design decisions such as the functional form of the cost function and the amount of liquidity in the market. We consider a specific model in which traders have exponential utility and exponential-family beliefs representing noisy estimates of ground truth. In this setting, sampling error vanishes as the number of traders grows, but there is a tradeoff between the other two components. We provide both upper and lower bounds on market-maker bias and convergence error, and demonstrate via numerical simulations that these bounds are tight. Our results yield new insights into the question of how to set the market's liquidity parameter and into the forecasting benefits of enforcing coherent prices across securities.

==> app-factor-two.tex <==
\section{Convergence Comparison of \IND and \LMSR}

\begin{lemma}
\label{lem:two:conv}
Let $\bprice\in\R^K$ be a probability vector with non-zero entries, let $H\coloneqq\parens{\diag_{k\in[K]}\price_k}-\bprice\bprice\trans$ be the covariance
matrix
of the associated multinomial distribution, and $D\coloneqq\diag_{k\in[K]}\price_k(1-\price_k)$ be the
diagonal matrix consisting of the diagonal of $H$. Let $\cL\coloneqq\range(D^{-1/2} H D^{-1/2})$. Then,
for any $\bu\in\cL$,
\[
  \bu\trans\bu
  \le \bu\trans D^{-1/2} H D^{-1/2} \bu
  \le 2\bu\trans\bu
\enspace.
\]
\end{lemma}
\begin{remark}
This implies that $1\le\lambda_{\min}(D^{-1/2} H D^{-1/2})$ and $\lambda_{\max}(D^{-1/2} H D^{-1/2})\le 2$. Thus, by \Eq{lambda:commute},
we also have $1\le\lambda_{\min}(H^{1/2}D^{-1}H^{1/2})$ and $\lambda_{\max}(H^{1/2}D^{-1}H^{1/2})\le 2$.
\end{remark}
\begin{proof}
Let $\bu\in\cL$ and $\bv=D^{-1/2}\bu$. To prove the lemma, we need to show that
\[
  \bv\trans D\bv
  \le \bv\trans H \bv
  \le 2\bv\trans D\bv
\enspace.
\]

\paragraph{Part 1: $\bv\trans D\bv\le \bv\trans H\bv$.}
We first rewrite the constraint $\bu\in\cL$ in terms of $\bv$.
%We begin by making the description of $\cL$ more explicit.
To start, note that $\bu\in\cL=\range(D^{-1/2} H D^{-1/2})$ iff
$\bu\perp\Null(D^{-1/2} H D^{-1/2})$. Next, note that $\by\in\Null(D^{-1/2} H D^{-1/2})$ iff $D^{-1/2}\by\in\Null(H)$,
which is equivalent to $\by\in D^{1/2}\Null(H)$. Now, $\Null(H)=\set{c\one:\:c\in\R}$, where $\one$ is the all-ones vector.
So,
\[
  \Null(D^{-1/2} H D^{-1/2})=D^{1/2}\Null(H)=\BigSet{\by:\: y_j=c\sqrt{\mu_j(1-\mu_j)} \text{ for $j\in[K]$, for some $c\in\R$}}
\enspace.
\]
Therefore, $\bu\perp\Null(D^{-1/2} H D^{-1/2})$ iff
%
\begin{equation}
\label{eq:L:explicit}
  \sum_{j\in[K]} u_j\sqrt{\mu_j(1-\mu_j)}=0
\enspace.
\end{equation}
%
Since $\bv=D^{-1/2}\bu$, we have $\bu=D^{1/2}\bv$, i.e., $u_j=v_j\sqrt{\mu_j(1-\mu_j)}$ for $j\in[K]$. Substituting this expression
into \Eq{L:explicit} yields
%
\begin{equation}
\label{eq:v:constr}
  \sum_{j\in[K]} v_j\mu_j(1-\mu_j)=0
\enspace.
\end{equation}
%
When $K=1$, then $D=H=\zero$, so in this case indeed $\bv\trans D\bv\le \bv\trans H\bv$. Next consider $K>1$. We will use the following
identity for $v_1\mu_1$, implied by \Eq{v:constr}:
%
\begin{equation}
\label{eq:v1}
  v_1\mu_1=-\frac{1}{1-\mu_1}\sum_{j\ge 2} v_j\mu_j(1-\mu_j)
\enspace.
\end{equation}
%
We next argue that $\bv\trans H\bv-\bv\trans D\bv\ge 0$:
%
\begin{align}
\label{eq:twoc:1}
\bv\trans H\bv-\bv\trans D\bv
  &=-\sum_{ \substack{j,k\in[K] \\ j\ne k} }
    \mu_j\mu_k v_j v_k
\\[2pt]
\notag
  &=-\sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    \mu_j\mu_k v_j v_k
    -2\sum_{k\ge 2}\mu_1 v_1 \mu_k v_k
\\
\label{eq:twoc:2}
  &=-\sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    \mu_j\mu_k v_j v_k
    +\frac{2}{1-\mu_1}\sum_{j,k\ge 2}\mu_j(1-\mu_j) v_j \mu_k v_k
\\
\label{eq:twoc:3}
  &=-\sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    z_j z_k
    +\frac{2}{1-\mu_1}\sum_{j,k\ge 2}(1-\mu_j) z_j z_k
\\
\label{eq:twoc:4}
  &=-\sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    z_j z_k
    +\frac{1}{1-\mu_1}\sum_{j,k\ge 2}\bigParens{(1-\mu_j)+(1-\mu_k)} z_j z_k
\\[2pt]
\notag
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    \sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    z_j z_k
    \BigParens{
     -(1-\mu_1)+(1-\mu_j)+(1-\mu_k)
    }
    +
    \sum_{j\ge 2}
    2(1-\mu_j)z_j^2
    \;}
\\[2pt]
\notag
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    \sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    z_j z_k
    \BigParens{
     (1-\mu_1-\mu_j-\mu_k)+2\mu_1
    }
    +
    \sum_{j\ge 2}
    z_j^2
    \BigParens{
     2(1-\mu_1-\mu_j) + 2\mu_1
    }
    \;}
\\[2pt]
\notag
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    2\mu_1\sum_{j,k\ge 2}
    z_j z_k
    +
    \sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    (1-\mu_1-\mu_j-\mu_k)
    z_j z_k
    +
    \sum_{j\ge 2}
    2(1-\mu_1-\mu_j) z_j^2
    \;}
\\[2pt]
\label{eq:twoc:5}
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    2\mu_1\sum_{j,k\ge 2}
    z_j z_k
    +
    \sum_{ \substack{j,k\ge 2 \\ j\ne k} }
    \sum_{ \substack{\ell\ge 2\\ \ell\ne j,k} }
    \mu_\ell
    z_j z_k
    +
    \sum_{j\ge 2}
    \sum_{ \substack{\ell\ge 2\\ \ell\ne j} }
    2\mu_\ell z_j^2
    \;}
\\[2pt]
\notag
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    2\mu_1\sum_{j,k\ge 2}
    z_j z_k
    +
    \sum_{ j,k\ge 2 }
    \sum_{ \substack{\ell\ge 2\\ \ell\ne j,k} }
    \mu_\ell
    z_j z_k
    +
    \sum_{j\ge 2}
    \sum_{ \substack{\ell\ge 2\\ \ell\ne j} }
    \mu_\ell z_j^2
    \;}
\\[2pt]
\notag
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    2\mu_1\sum_{j,k\ge 2}
    z_j z_k
    +
    \sum_{ \ell\ge 2 }
    \mu_\ell
    \!\!\sum_{ \substack{j,k\ge 2 \\ j\ne\ell,k\ne\ell} }\!\!
    z_j z_k
    +
    \sum_{j\ge 2}
    \sum_{ \substack{\ell\ge 2\\ \ell\ne j} }
    \mu_\ell z_j^2
    \;}
\\[2pt]
\label{eq:twoc:6}
  &=\frac{1}{1-\mu_1}
    \BigBracks{\;
    2\mu_1\BigParens{\sum_{j\ge 2}z_j}^2
    +
    \sum_{ \ell\ge 2 }
    \mu_\ell
    \BigParens{\sum_{\substack{j\ge 2\\j\ne\ell}} z_j}^2
    +
    \sum_{ \substack{j,\ell\ge 2\\ \ell\ne j} }
    \mu_\ell z_j^2
    \;}
  \ge 0
\enspace.
\end{align}
%
In \Eq{twoc:1}, we use the fact that $D$ is the diagonal of $H$, so the right-hand side only sums over off-diagonal entries of $H$.
In \Eq{twoc:2}, we replaced $\mu_1 v_1$ using \Eq{v1}. In \Eq{twoc:3}, introduce the substitution $z_j\coloneqq \mu_j v_j$.
In \Eq{twoc:4}, we use the fact that $2\sum_{j,k\ge 2}(1-\mu_j)z_j z_k=\sum_{j,k\ge 2}(1-\mu_j)z_j z_k+\sum_{j,k\ge 2}(1-\mu_k)z_j z_k$.
In \Eq{twoc:5}, we use the fact that $\sum_{\ell\in[K]}\mu_\ell=1$ and so $(1-\mu_1-\mu_j-\mu_k)=\sum_{\ell\ne 1,j,k}\mu_\ell$
and $(1-\mu_1-\mu_j)=\sum_{\ell\ne 1,j}\mu_\ell$.
Finally, the inequality in \Eq{twoc:6} follows because $\mu_1,\mu_\ell\ge 0$.

\paragraph{Part 2: $\bv\trans H\bv\le 2\bv\trans D\bv$.} We show by direct calculation that $2\bv\trans D\bv-\bv\trans H\bv\ge 0$:
%
\begin{align}
\label{eq:twoc:21}
2\bv\trans D\bv-\bv\trans H\bv\ge 0
  &=2\BigBracks{\;\sum_{j\in[K]}\mu_j v_j^2-\sum_{j\in[K]}\mu_j^2 v_j^2\;}
    -\BigBracks{\;\sum_{j\in[K]}\mu_j v_j^2-\sum_{j,k\in[K]}\mu_j\mu_k v_j v_k\;}
\\[4pt]
\notag
  &=\sum_{j\in[K]}\mu_j v_j^2-2\sum_{j\in[K]}\mu_j^2 v_j^2
    +\sum_{j,k\in[K]}\mu_j\mu_k v_j v_k
\\[4pt]
\label{eq:twoc:22}
  &=\sum_{j,k\in[K]}\mu_j\mu_k v_j^2-2\sum_{j\in[K]}\mu_j^2 v_j^2
    +\sum_{j,k\in[K]}\mu_j\mu_k v_j v_k
\\[4pt]
\notag
  &=\sum_{\substack{j,k\in[K]\\ j\ne k}} \mu_j\mu_k v_j^2
    +\sum_{\substack{j,k\in[K]\\ j\ne k}} \mu_j\mu_k v_j v_k
\\[2pt]
\label{eq:twoc:23}
  &=\sum_{\substack{j,k\in[K]\\ j\ne k}}\BigParens{\frac12 \mu_j\mu_k v_j^2+\frac12 \mu_j\mu_k v_k^2+\mu_j\mu_k v_j v_k}
\\
\label{eq:twoc:24}
  &=\sum_{\substack{j,k\in[K]\\ j\ne k}}\frac12\mu_j\mu_k\Parens{v_j+v_k}^2
  \ge 0
\enspace.
\end{align}
In \Eq{twoc:21}, we just use the definition of $H$ and $D$. In \Eq{twoc:22}, we use that $\sum_{k\in[K]}\mu_k=1$. In \Eq{twoc:23},
we use that by symmetry $\sum_{j\ne k} \mu_j\mu_k v_j^2=\sum_{j\ne k} \mu_j\mu_k v_k^2$ and so $\sum_{j\ne k} \mu_j\mu_k v_j^2=\sum_{j\ne k} \mu_j\mu_k (v_j^2+v_k^2)/2$.
The final inequality in \Eq{twoc:24} follows because $\mu_j,\mu_k\ge 0$.
\end{proof}


==> sampling.tex <==
\section{Sampling Error and the Risk-Aversion Effect}
\label{sec:sampling}
\label{SEC:SAMPLING} % so we can reference in appendix section title

The market's forecasting ability is fundamentally limited by the information present
among the population of traders, and the traders' risk attitudes in
communicating their information via trades. In this section, we
quantify these sources of error by analyzing the discrepancy
$\norm{\bpricetruth - \aggbprice}$ between the true expected
security values and the market-clearing equilibrium prices; here,
$\norm{\cdot}$ denotes the standard Euclidean norm.
The
following characterization of $\aggbprice$ allows
us to bound this discrepancy.
%
\begin{theorem}\label{thm:eqprice-char}
  Under the exponential trader model, the unique market-clearing
  equilibrium prices $\aggbprice$ can be written as
\vspace{-5pt}
  \begin{equation}
    \label{eq:price-eq-form}
 \aggbprice =
 \nabla \lmsr\Parens{
 \frac{\sum_{i=1}^\nbuyers \bttheta_i/a_i}
      {\sum_{i=1}^\nbuyers 1/a_i}
 }
\enspace.
  \end{equation}
\end{theorem}

This form %of the price equilibrium in~(\ref{eq:price-eq-form})
 reflects
two possible sources of error. First, the beliefs
$\bttheta_i$ are typically noisy signals of the ground truth. Second,
beliefs are weighted according to risk aversions $a_i$, which can skew
the prices. To formalize the latter
concept, we write
%
$\Neff = \Parens{\sum_i a_i^{-1}}^2 / \Parens{\sum_i a_i^{-2}}$
%
to denote the \emph{effective sample size} of the weighted average.
When risk aversion coefficients are equal across agents, we have $\Neff = N$, and
when one agent has much smaller risk aversion than the others,
$\Neff \rightarrow 1$. As the next result shows, the magnitude of the
sampling error depends on the effective sample size as it relates to
the number of securities and the variance in trader beliefs.
%
\begin{theorem}\label{thm:sampling-error}
  Under the exponential trader model, assume that the beliefs
  $\bttheta_i$ are drawn independently for each trader $i \in [N]$
  with mean $\exNoBrack[\bttheta_i] = \btheta^\TRUE$ and covariance
  $\varNoBrack(\bttheta_i) \preceq \sigma^2 I_K$ for some $\sigma^2 \geq 0$.
  For any $\delta \in (0,1)$, the market-clearing prices $\aggbprice$
  satisfy, with probability at least $1 - \delta$,
$
\norm{\aggbprice - \bpricetruth} \leq
O\left(\, \sigma \sqrt{K/(\Neff\,\delta)} \,\right).
$
Furthermore, assuming that each $a_i$ lies in a bounded range
$(a_{\min}, a_{\max})$ where $a_{\min}, a_{\max} > 0$,
we have that $\Neff \rightarrow \infty$ as $N \rightarrow \infty$.
\label{thm:Neff}
\end{theorem}
%
To interpret this result, note that the characterization of
market-clearing prices in~\eqref{eq:aggbdual} evokes standard
statistical estimators such as the maximum likelihood estimate (after
rescaling the objective by $1/N$). Theorem~\ref{thm:sampling-error}
implies that as the number of traders grows large, the market prices
$\aggbprice$ converge to the ground truth $\bpricetruth$ in
probability. It is important to note that this relies on
Theorem~\ref{thm:eqprice-char}, which is an artifact of exponential
utility---for general utilities, market-clearing prices may not be
consistent in the statistical sense, and this extra discrepancy would
need to be quantified.

For a finite number of traders, the bound in
Theorem~\ref{thm:sampling-error} increases with the belief variance
and the number of securities, as one would expect. It decreases with
the effective sample size: the information incorporated into
market-clearing prices improves when risk aversions are more uniform, and when the number of agents increases. 

%\jenn{Cut this sentence for space, may want it back in final version.}
\ignore{
We stress that
the distributional assumptions of the theorem are only needed to bound
the sampling error, and are not required in the remainder of the
paper, which deals with sources of error once traders' beliefs have
been drawn and fixed.
}
